Attack of the Tails: Yes, You Really Can Backdoor Federated Learning

Due to its decentralized nature, Federated Learning (FL) lends itself to adversarial attacks in the form of backdoors during training. The goal of a backdoor is to corrupt the performance of the trained model on specific sub-tasks (e.g., by classifying green cars as frogs). A range of FL backdoor attacks have been introduced in the literature, but also methods to defend against them, and it is currently an open question whether FL systems can be tailored to be robust against backdoors. In this work, we provide evidence to the contrary. We first establish that, in the general case, robustness to backdoors implies model robustness to adversarial examples, a major open problem in itself. Furthermore, detecting the presence of a backdoor in a FL model is unlikely assuming first order oracles or polynomial time. We couple our theoretical results with a new family of backdoor attacks, which we refer to as edge-case backdoors. An edge-case backdoor forces a model to misclassify on seemingly easy inputs that are however unlikely to be part of the training, or test data, i.e., they live on the tail of the input distribution. We explain how these edge-case backdoors can lead to unsavory failures and may have serious repercussions on fairness, and exhibit that with careful tuning at the side of the adversary, one can insert them across a range of machine learning tasks (e.g., image classification, OCR, text prediction, sentiment analysis).

==> BroderImpacts.tex <==
%!TEX root = edge_case_attack_neurips20.tex
\section{Broader Impacts}
% this is a copy paste from the intro. DONT LEAVE AS IS

Federated Learning has been proposed recently as a new paradigm to train predictive models on heterogeneous user data, so that applications like personal assistants can be more personalized, while simultaneously ensuring user privacy. Because this technique is hypothesized to be deployed on millions or even billions of devices in the future, a tight scrutiny on all aspects of this framework is necessitated.

\paragraph{Fundamental security risk of FL} This work will bring in a broader impact to the FL community by alarming them of the existence of \textit{edge-case backdoors} and its implications. 
%potential to harm the whole federated learning systems.
%, which can be considered as a serious issue in the fairness of a system.
\textit{Edge-case} data refers to data points that reside on the tails of the input distribution, i.e., rare, but natural inputs. 
\textit{Edge-case backdoors} are attacks that target such data points and force them to be misclassified by the predictive global model.
We present concrete examples of such \textit{backdoors}, ranging from image classification tasks to next word prediction, and demonstrate that edge-case backdoors can be easily hard-wired to FL models.
These backdoors can further bypass state-of-the-art defense mechanisms proposed in the literature.
More worryingly, since they do not affect the majority of the data, they tend to go unnoticed, especially when the metrics which test the quality of the system look at aggregate performance measures.
This problem is unfortunately not new, and there have been incidents in the past that have brought it to light~\cite{WhenItComesTom2018}. In autonomous vehicles, \textit{backdoor} attacks have been known to compromise security~\cite{TeslaAndrew2019, TheveryhumanKrafcik2018}.

% The \textit{edge-case backdoors} can also manifest in the form of non-fairness related problems such as those which compromise the security of autonomous vehicles \cite{TeslaAndrew2019,TheveryhumanKrafcik2018}

\paragraph{Unfair treatment of users} 
%In this work, we show systematically how the current FL framework is indeed vulnerable to \textit{edge-case backdoor} attacks. 
%Our theoretical justification shows that ensuring \textit{backdoor} robustness is difficult to achieve in general, and follow it up with extensive experiments on various vision and language tasks to give sufficient empirical evidence to support our claims.
The second aspect of our work highlights that any attempts to improve the security of FL systems may result in an unfair treatment of the clients served.
That is, secure FL may successfully defend backdoor attacks, but it may also filter out users that generate diverse data sets.
This leads to an alarming fairness countereffect with regards to robustness.
This demonstrates a largely unexplored fairness and robustness trade-off which has already been highlighted in \cite{kairouz2019advances}.
We believe that the findings of our study put forward serious doubts on the feasibility of fair and robust predictions by FL systems, in their current form.


In summary, the impact of our work is to question the robustness, security, and fairness guarantees of FL system providers, and present several important challenges to the related research community.
% has to seriously rethink how to guarantee robust and fair predictions in the presence of edge-case failures.
